Enhancing Model Robustness and Fairness with Causality: A Regularization Approach

Recent work has raised concerns on the risk of spurious correlations and unintended biases in statistical machine learning models that threaten model robustness and fairness. In this paper, we propose a simple and intuitive regularization approach to integrate causal knowledge during model training and build a robust and fair model by emphasizing causal features and de-emphasizing spurious features. Specifically, we first manually identify causal and spurious features with principles inspired from the counterfactual framework of causal inference. Then, we propose a regularization approach to penalize causal and spurious features separately. By adjusting the strength of the penalty for each type of feature, we build a predictive model that relies more on causal features and less on non-causal features. We conduct experiments to evaluate model robustness and fairness on three datasets with multiple metrics. Empirical results show that the new models built with causal awareness significantly improve model robustness with respect to counterfactual texts and model fairness with respect to sensitive attributes.

==> comments.tex <==
============================================================================
                            REVIEWER #1
============================================================================

---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                   Appropriateness (1-5): 4
                           Clarity (1-5): 4
      Originality / Innovativeness (1-5): 3

Detailed Comments
---------------------------------------------------------------------------
This paper proposes a regularization approach to improve model robustness and fairness. The main idea is to first identify features as either causal or spurious (or neither), and then regularize these groups differently, such that non-causal features are penalized more. In practice, this is done by manually inspecting (a subset of) the features, splitting them into groups, and introducing different regularization hyper-parameters for each group. The experiments are done on two text classification datasets and one law school admissions dataset, and yield improvements in robustness (in the first case) and fairness (in the admissions case) as measured on counterfactual test sets. 

The high-level approach proposed by the paper is intuitive and simple, and hence attractive. The main concerns I have are three:
1. The process of identifying spurious and causal features is not well described, and is not generalizable to other settings. See more on this below. 
2. The experiments include hyper-parameter tuning of the regularization parameters, but it is not clear if the hyper-params were tuned in-distribution or out of distribution. This is crucial for experiments with robustness and fairness. See more on this below. 
3. The law school admissions dataset is not a text processing data at all. This isn't necessarily a bad thing, but it doesn't qualify as a fairness dataset in NLP, and once you're out of the NLP world, there may be other datasets that are more appropriate, with which I'm not familiar. 

I still think the paper presents an interesting idea, but the (first two) issues above are potential pretty serious problems. 


Major issues:
=============
1. Identifying spurious and causal features: this is a key step, but is described very briefly. From what I could tell (section 4.1), the authors manually split features into spurious and causal. That may be ok for the law school admissions dataset (low-dimensional), but it's not clear how it is done for the text datasets. Later, section 5.2 gives a bit more information: a binary classifier was trained, supposedly on a bag-of-words representation of the texts. The features that were assigned the highest weights in this classifier are passed to two annotators who split them into causal and spurious; they also add more causal features from the whole vocabulary. In the admissions dataset, gender is furious but race is not (not sure if this means it's not used at all or just not considered furious; and if so, how is race used if at all?). 
There are several potential problems with this setup:
a. First, more details are necessary about the process of identifying causal features. Section 4.1 mentions high annotation agreement, but it's not clear which dataset this refers to. Who are the annotators and what were the instructions given to them? How many features were considered in total as "top coefficient" and why does the threshold make sense? Is there some characterizations of the features that makes sense? Like, certain POS tags that are identified as spurious vs causal?
b. Second, this feature identification process is limited to a certain text representation (sparse bag of words) and classifier (linear). How could this be generalized to other representations and classifiers? Section 6.2 discusses extensions to deep classifiers, but those still assumes a split into spurious and causal features. 

2. Regularization penalties end up being large on non-causal features and small on causal features, which is intuitive. I'm not sure how the hyper-parameter tuning was done though. If it was done on the (in-distribution) validation set, then this result would be surprising, as in distribution the spurious features are also helpful (that's the whole problem). If hyper-parameter tuning was done on o.o.d data, then it can no longer be said that no such data was used at training time. This is the problem of model selection, which does not have an easy solution. But I'd expect at least a more clear description and discussion of this issue, and the effect of how hyper-param tuning is done on the results.
---------------------------------------------------------------------------


Questions for Authors
---------------------------------------------------------------------------
- The paper mentions fairness concepts (individual, group, max-min), without defining or explaining them. 
- The proposed approach is argued to be explainable. However, it's tricky to interpret larger weights and more important, if that's what is meant by explainable. 
- The law school admissions dataset is mentioned early on but not referenced until later in a footnote. In fact, it isn't a text processing dataset (inputs and labels are categorical).
- - Experiments with two text classification datasets (rather small) and one school admissions dataset (low-dimensional categorical variables, not text).  The IMDB dataset comes with a counterfactual test set; for the Kindle one the authors create a counterfactual test set. There are very little details about this procedure. 
- The approach is compared with other regularizations, but not with prior approaches. Even though the authors explain that other approaches are not comparable as they use more information, it would be good to at least provide such numbers as an upper bound for comparison.
---------------------------------------------------------------------------



============================================================================
                            REVIEWER #2
============================================================================

---------------------------------------------------------------------------
Reviewer's Scores
---------------------------------------------------------------------------
                   Appropriateness (1-5): 4
                           Clarity (1-5): 5
      Originality / Innovativeness (1-5): 3

Detailed Comments
---------------------------------------------------------------------------
The authors present a regularization approach for improving the robustness of text classifiers. The identify causal features (n-gram words) in the corpus and impose penalties on the causal/spurious/remaining features by imposing regularization based on the respective feature weights in the loss objective. Their approach yields significant improvements over Logistic Regression baselines (with and without word embeddings), which is promising. However, there are some gaps in the paper that need to be addressed. Please see comments and questions below:

Lines 312-320: More details are needed on the annotation process for identifying spurious features. How many annotators were there? Did they go through the entire corpus, sample by sample, or were they presented the top K features from which the spurious vs. causal features were selected?
Line 372-373: I think the goal here should be to train a model that generalizes better to unseen data i.e. validation or test set, rather than maximizing performance on training set, as the latter can be easily achieved with overfitting.
Line 331 - convert to in-line citation
Line 337-capitalize L in l1/l2 for clearer reading
Lines 475-478: I don't agree with the statement that this approach does not need to be compared to data augmentation, since annotations were carried out to identify the casual/spurious features and integrate them into the loss function while training. In a way, this approach does involve data augmentation, just not in the conventional way. In any case, it would be useful to observe results from counterfactual data augmentation in tandem with this approach.
Lines 612: assign -> assigning
Section 6.2: This section is a good start on how the approach could be transferred to the deep learning framework. A preliminary experiment along these lines will make the paper much stronger.
---------------------------------------------------------------------------


% \begin{table*}
%     \centering \small
%     \begin{tabular}{l| l l l | l l l} 
%     \hline
%       & \multicolumn{3}{c|}{{\bf IMDB}} & \multicolumn{3}{c}{{\bf Kindle}} \\
%          \cline{2-7}
        
%          {\bf Penalty} & {\bf $\lambda_c,\lambda_s,\lambda_r$} & {\bf Test} & {\bf CTF} & {\bf $\lambda_c,\lambda_s,\lambda_r$} & {\bf Test} & {\bf CTF} \\
%          \hline
%          LR+l2 (BOW) & (1,1,1) & 0.845 $\pm$ 0.005 & 0.567 $\pm$ 0.009 & (1,1,1) & 0.853 $\pm$ 0.027 & 0.412 $\pm$ 0.048 \\
%          LR(Glove) & N/A & 0.824 $\pm$ 0.002 & 0.619 $\pm$ 0.006 & (1,1,1) & 0.820 $\pm$ 0.004 & \cellcolor{brown!30}{0.553 $\pm$ 0.027} \\
%          Feature selection & (1,1,1) & 0.835 $\pm$ 0.005 & \cellcolor{brown!30}{0.633 $\pm$ 0.012} & (1,1,1) & 0.850 $\pm$ 0.002 & 0.510 $\pm$ 0.017 \\ 
%          %; 
         
%         %  \notezw{LSTM (AAAI)} & Null & 0.811 & 0.700 & Null & 0.908 & 0.642 \\
%          \hline
%          causal+spurious & (0,10,0) & 0.836 $\pm$ 0.006 & 0.632 $\pm$ 0.005 & (0,10,0) & 0.857 $\pm$ 0.007 & 0.545 $\pm$ 0.013\\
%          causal+non-causal & (0,100,100) & 0.821 $\pm$ 0.011 & \cellcolor{brown!30}{0.658 $\pm$ 0.01} & (0,10,10) & 0.843 $\pm$ 0.003 & 0.557 $\pm$ 0.003 \\
%          causal+spurious+remain & (0,100,0.1) & 0.841 $\pm$ 0.007 & 0.635 $\pm$ 0.006 & (0,100,1) & 0.847 $\pm$ 0.003 & \cellcolor{brown!30}{0.571 $\pm$ 0.008} \\
%          \hline
%          LR+l2 (BOW) & (1,1,1) & 0.845 $\pm$ 0.003 & 0.567 $\pm$ 0.005 & (1,1,1) & 0.874 $\pm$ 0.006 & 0.452 $\pm$ 0.021 \\
%         %  \notezw{LSTM (baseline)} & & & & & & \\
%          causal+spurious & (0,10,0) & 0.838 $\pm$ 0.004 & 0.634 $\pm$ 0.007 & (0,100,0) & 0.857 $\pm$ 0.003 & 0.545 $\pm$ 0.01\\
%          causal+non-causal & (0,100,100) & 0.843 $\pm$ 0.005 & \cellcolor{brown!30}{0.700 $\pm$ 0.007} & (0,10,10) & 0.855 $\pm$ 0.005 & \cellcolor{brown!30}{0.641 $\pm$ 0.006} \\
%          causal+spurious+remain & (0.01,100,100) & 0.840 $\pm$ 0.004 & \cellcolor{brown!30}{0.697 $\pm$ 0.008} & (0.001,1,10) & 0.848 $\pm$ 0.006 & \cellcolor{brown!30}{0.636 $\pm$ 0.003} \\
%          \hline
         
%     \end{tabular}
%     \caption{Robustness evaluation for tuned classifiers. Accuracy reported for test and Counterfactual (CTF) data from IMDB and Kindle dataset. Results in 1st section are baselines, 2nd section are based on causal features identified from top coefficient terms and 3rd section are based on causal features identified from the whole vocabulary.\notezw{clear}}
%     \label{tab.CTF_robust}
% \end{table*} 

